Towards Tactile Internet in Beyond 5G Era: Recent Advances, Current Issues and Future Directions

Tactile Internet (TI) is envisioned to create a paradigm shift from the content-oriented communications to steer/control-based communications by enabling real-time transmission of haptic information (i.e., touch, actuation, motion, vibration, surface texture) over Internet in addition to the conventional audiovisual and data traffics. This emerging TI technology is expected to create numerous opportunities for technology markets in a wide variety of applications ranging from teleoperation systems and AR/VR to automotive safety and eHealthcare towards addressing the complex problems of human society. However, the realization of TI over wireless media in the upcoming 5G and beyond networks creates various non-conventional communication challenges and stringent requirements. To this end, this paper aims to provide a holistic view on wireless TI along with a thorough review of the existing literature, to identify and analyze the involved technical issues, to highlight potential solutions and to propose future research directions. First, starting with the vision of TI and recent advances and a review of related survey/overview articles, we present a generalized framework for wireless TI in the Beyond 5G Era including a TI architecture, main technical requirements, key application areas and potential enabling technologies. Subsequently, we provide a comprehensive review of the existing TI works by broadly categorizing them into three main paradigms; namely, haptic communications, wireless AR/VR, and autonomous, intelligent and cooperative mobility systems. Next, potential enabling technologies across physical/MAC and network layers are identified and discussed in detail. Also, security and privacy issues of TI applications are discussed along with some promising enablers. Finally, we present some open research challenges and recommend promising future research directions.

==> HEADERSETUP.latex <==
\pagestyle{fancyplain}
\renewcommand{\chaptermark}[1]%
                       {\markboth{#1}{}}
\renewcommand{\sectionmark}[1]%
                       {\markright{\thesection\ #1}}
\lhead[\fancyplain{}{\bfseries\thepage}]
     {\fancyplain{}{\bfseries\rightmark}}
\rhead[]{} \cfoot[\fancyplain{}{\bfseries\thepage}]{\fancyplain{}{\bfseries\thepage}}
\newpage

